Single-Shot Domain Adaptation via Target-Aware Generative Augmentation

The problem of adapting models from a source domain using data from any target domain of interest has gained prominence, thanks to the brittle generalization in deep neural networks. While several test-time adaptation techniques have emerged, they typically rely on synthetic data augmentations in cases of limited target data availability. In this paper, we consider the challenging setting of single-shot adaptation and explore the design of augmentation strategies. We argue that augmentations utilized by existing methods are insufficient to handle large distribution shifts, and hence propose a new approach SiSTA (Single-Shot Target Augmentations), which first fine-tunes a generative model from the source domain using a single-shot target, and then employs novel sampling strategies for curating synthetic target data. Using experiments with a state-of-the-art domain adaptation method, we find that SiSTA produces improvements as high as 20\% over existing baselines under challenging shifts in face attribute detection, and that it performs competitively to oracle models obtained by training on a larger target dataset.

==> sections/related.tex <==
\section{Related Works}
\label{sec:related}
The problem of distribution shift 
\begin{itemize}
    \item Image space augmentation based techniques
    \item Feature space augmentation
\end{itemize}

\textbf{GAN based domain adaptation:}
    \citep{morerio2020generative} deploys a conditional GAN trained on target dataset with noisy pseudo labels generated by the source model to generate clean target distribution. Approaches like \citep{sankaranarayanan2018generate} \citep{hu2018duplex} \citep{hoffman2018cycada} aim at bringing the source and target distribution closer in a learned joint feature space, such methods depend on the availability of both source and target distribution. Few GAN based strategies \citep{gal2021stylegan} \citep{zhu2021mind} have been proposed for few-shot domain adaptation tasks, both of these solutions utilize CLIP a multi-modal(language and visual) encoder to model the domain gap.  \citep{yang2020one} proposes 
